Aligning Instruction Tasks Unlocks Large Language Models as Zero-Shot Relation Extractors

Recent work has shown that fine-tuning large language models (LLMs) on large-scale instruction-following datasets substantially improves their performance on a wide range of NLP tasks, especially in the zero-shot setting. However, even advanced instruction-tuned LLMs still fail to outperform small LMs on relation extraction (RE), a fundamental information extraction task. We hypothesize that instruction-tuning has been unable to elicit strong RE capabilities in LLMs due to RE's low incidence in instruction-tuning datasets, making up less than 1% of all tasks (Wang et al., 2022). To address this limitation, we propose QA4RE, a framework that aligns RE with question answering (QA), a predominant task in instruction-tuning datasets. Comprehensive zero-shot RE experiments over four datasets with two series of instruction-tuned LLMs (six LLMs in total) demonstrate that our QA4RE framework consistently improves LLM performance, strongly verifying our hypothesis and enabling LLMs to outperform strong zero-shot baselines by a large margin. Additionally, we provide thorough experiments and discussions to show the robustness, few-shot effectiveness, and strong transferability of our QA4RE framework. This work illustrates a promising way of adapting LLMs to challenging and underrepresented tasks by aligning these tasks with more common instruction-tuning tasks like QA.

==> tables/instruction-discussion.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
\small
\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{\textbf{LLMs}} & \multirow{2}{*}{\textbf{I-T}} & \multirow{2}{*}{\textbf{RLHF}} & \multirow{2}{*}{\textbf{C-T}} & \multicolumn{3}{c}{\textbf{Avg. F1}} \\
                               &                               &                                &                               & Vanilla    & QA4RE            & $\Delta$ \\ \midrule
% \multicolumn{4}{c}{Random Gussing}                                                                                              & \multicolumn{2}{c}{18.2}      & -        \\ \midrule
% davinci                        &                               &                                &                               & 21.5       & 20.5             & -1.0     \\
% t-d-1                          & $\checkmark$                  &                                &                               & 23.0       & 15.3             & -7.7     \\
% c-d-2                          & $\checkmark$                  &                                & $\checkmark$                  & 39.2       & 47.8             & 8.6      \\
% t-d-2                          & $\checkmark$                  &                                & $\checkmark$                  & 43.7       & 46.8             & 3.1      \\
% t-d-3                          & $\checkmark$                  & $\checkmark$                   & $\checkmark$                  & 48.1       & \textbf{59.4}    & 11.3     \\ \bottomrule
\multicolumn{1}{l}{davinci}      &                               &                                &                               & 23.6          & 23.7       & \textcolor{ForestGreen}{$+$0.1}         \\
% davinci                        &                               &                                &                               & 23.6          & 23.7       & 0.1         \\

\multicolumn{1}{l}{text-001}     & $\checkmark$                  &                                &                               & 22.3          & 14.9       & \textcolor{WildStrawberry}{$-$7.4}        \\
\multicolumn{1}{l}{code-002}     & $\checkmark$                  &                                & $\checkmark$                  & 39.8          & 43.9       & \textcolor{ForestGreen}{$+$4.1}         \\
\multicolumn{1}{l}{text-002}     & $\checkmark$                  &                                & $\checkmark$                  & 43.2          & 45.9       & \textcolor{ForestGreen}{$+$2.7}         \\
\multicolumn{1}{l}{text-003}     & $\checkmark$                  & $\checkmark$                   & $\checkmark$                  & 47.6          & 55.8       & \textcolor{ForestGreen}{$+$8.2}  \\
\multicolumn{1}{l}{ChatGPT}      & $\checkmark$                  & $\checkmark$                   & $\checkmark$                  & 40.1          & 46.0       & \textcolor{ForestGreen}{$+$5.9}  \\
\bottomrule
\end{tabular}
}
\caption{Effectiveness of our QA4RE frameworks on GPT-3.5 series LLMs with different pre-training/fine-tuning strategies (\%).
I-T, RLHF, and C-T refer to Instruction-Tuning, Reinforcement Learning with Human Feedback, and Code-Tuning, respectively.
}
\label{tab:instruction-discussion}
\vspace{-5pt}
\end{table}

==> tables/t5_size_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
\small
\centering
% \resizebox{0.47\textwidth}{!}{
% \begin{tabular}{lcccccc}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{FLAN-T5 Size}}} & \multicolumn{3}{c}{\textbf{Avg. F1}}                               \\
% \multicolumn{1}{c}{}                                       & Vanilla          & QA4RE          & $\Delta$ \\ \midrule
% % Small                                                      & 19.5             & 25.0           & \textcolor{ForestGreen}{$+$5.6}                            \\
% % Base                                                       & 22.3             & 26.4           & \textcolor{ForestGreen}{$+$4.2}                            \\
% % Large                                                      & 34.8             & 41.8           & \textcolor{ForestGreen}{$+$7.0}                            \\
% % XLarge                                                     & 46.6             & 54.3           & \textcolor{ForestGreen}{$+$7.7}                        \\
% % XXLarge                                                    & 46.5             & 55.1           & \textcolor{ForestGreen}{$+$8.6}                            \\ 

% Small                                                      & 18.1             & 23.7           & \textcolor{ForestGreen}{$+${5.6}} \\
% Base                                                       & 19.8             & 25.9           & \textcolor{ForestGreen}{$+${6.2}} \\
% Large                                                      & 33.5             & 40.5           & \textcolor{ForestGreen}{$+${7.1}} \\
% XLarge                                                     & 45.3             & 52.9           & \textcolor{ForestGreen}{$+${7.7}} \\
% XXLarge                                                    & 45.2             & 53.9           & \textcolor{ForestGreen}{$+${8.7}} \\
% \bottomrule


% \end{tabular}

% \begin{tabular}{llccccc}
\begin{tabular}{llccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{FLAN-T5 Size}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Params}}} & \multicolumn{3}{c}{\textbf{Avg. F1}}                                                                                               \\
\multicolumn{1}{c}{}                                       & \multicolumn{1}{c}{}                                   & Vanilla          & QA4RE          & $\Delta$ \\ \midrule
Small                                                      & 80M                                                    & 18.1             & 23.7           & \textcolor{ForestGreen}{$+${5.6}} \\
Base                                                       & 250M                                                   & 19.8             & 25.9           & \textcolor{ForestGreen}{$+${6.2}} \\
Large                                                      & 780M                                                   & 33.5             & 40.5           & \textcolor{ForestGreen}{$+${7.1}} \\
XLarge                                                     & 3B                                                     & 45.3             & 52.9           & \textcolor{ForestGreen}{$+${7.7}} \\
XXLarge                                                    & 11B                                                    & 45.2             & 53.9           & \textcolor{ForestGreen}{$+${8.7}} \\ \bottomrule
\end{tabular}

% }
\caption{Effectiveness of our QA4RE frameworks on FLAN-T5 series models with different sizes.
The results are averaged over the full test set of four RE datasets.
% For reference, we add random guessing results on type-constraint relation.
}
\label{tab:t5-sizes}
\vspace{-10pt}
\end{table}

==> tables/zero-shot-main-F1-only.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{cc|lllll}
\toprule
\multicolumn{2}{c|}{Datasets}                                   & \textbf{TACRED}                             & \textbf{RE-TACRED}                       & \textbf{TACREV}                            & \textbf{SemEval} & \multicolumn{1}{c}{\textbf{Avg.}}            \\ \midrule
\multicolumn{2}{c|}{NLI$_{\text{BART}}$~\cite{Sainz2021NLI}}    & {\ul 49.7}                                  & 44.0                                     & 50.4                                       & 22.6             & 41.7                                        \\
\multicolumn{2}{c|}{NLI$_{\text{RoBERTa}}$~\cite{Sainz2021NLI}} & 47.1                                        & 58.7                                     & 49.9                                       & 19.1             & 43.7                                        \\
\multicolumn{2}{c|}{NLI$_{\text{DeBERTa}}$~\cite{Sainz2021NLI}} & 49.4                                        & \textbf{64.3}                            & 49.6                                       & 23.7             & 46.8                                        \\
\multicolumn{2}{c|}{SuRE$_\text{BART}$~\cite{Lu2022SuRE}}       & 20.4                                        & 23.6                                     & 22.2                                       & 0.0              & 16.5                                        \\
\multicolumn{2}{c|}{SuRE$_\text{PEGASUS}$~\cite{Lu2022SuRE}}    & 21.8                                        & 22.4                                     & 21.6                                       & 0.0              & 16.4                                        \\ \midrule
\multirow{2}{*}{text-davinci-002}            & Vanilla          & 43.7                                        & 55.9                                     & 43.3                                       & 30.1             & 43.2                                        \\
                                             & QA               & 46.8 (\textcolor{green}{$+$ 3.1})           & 56.5 (\textcolor{green}{$+$ 0.6})        & 48.8 (\textcolor{green}{$+$ 5.4})          & 31.6             & 45.9  (\textcolor{green}{$+$ 2.7})          \\
\multirow{2}{*}{code-davinci-002}            & Vanilla          & 39.2                                        & 53.1                                     & 40.6                                       & 26.4             & 39.8                                        \\
                                             & QA               & 47.8 (\textcolor{green}{$+$ 8.6})           & 58.2  (\textcolor{green}{$+$ 5.1})       & 42.7  (\textcolor{green}{$+$ 2.1})         & 27.0             & 43.9  (\textcolor{green}{$+$ 4.1})          \\
\multirow{2}{*}{text-davinci-003}            & Vanilla          & 48.1                                        & 55.3                                     & {\ul 51.0}                                 & {\ul 36.0}       & {\ul 47.6}                                  \\
                                             & QA               & \textbf{59.4} (\textcolor{green}{$+$ 11.3}) & {\ul 61.2}  (\textcolor{green}{$+$ 5.9}) & \textbf{59.4} (\textcolor{green}{$+$ 8.4}) & \textbf{43.3}    & \textbf{55.8}  (\textcolor{green}{$+$ 8.2}) \\ \bottomrule
\end{tabular}
}
\caption{}
\label{tab:main-table}
\end{table*}

==> tables/zero-shot-main-v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
% \small
\centering
\resizebox{\textwidth}{!}{
% \begin{tabular}{ll|lllllllllllll}
% \toprule
% % \multicolumn{2}{c|}{\multirow{2}{*}{Datasets}}                  & \multicolumn{3}{c}{\textbf{TACRED}}                                                         & \multicolumn{3}{c}{\textbf{RE-TACRED}}                                                   & \multicolumn{3}{c}{\textbf{TACREV}}                                                        & \multicolumn{3}{c}{\textbf{SemEval}}                                                        & \multicolumn{1}{c}{\textbf{Average}}            \\
% % \multicolumn{2}{c|}{}                                           & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                      & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                   & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                     & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                      & \multicolumn{1}{c}{F1}             \\ \midrule
% \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Methods}}}                  & \multicolumn{3}{l}{$\mspace{24mu}$ \textbf{TACRED}}                                                         & \multicolumn{3}{l}{$\mspace{10mu}$ \textbf{RE-TACRED}}                                                   & \multicolumn{3}{l}{$\mspace{24mu}$ \textbf{TACREV}}                                                        & \multicolumn{3}{l}{$\mspace{24mu}$ \textbf{SemEval}}                                                        & \multicolumn{1}{l}{$\mspace{1mu}$\textbf{Avg.}}            \\
% \multicolumn{2}{c|}{}                                           & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                      & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                   & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                     & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                      & \multicolumn{1}{l}{$\mspace{3mu}$ F1}             \\ \midrule
% \multicolumn{2}{l|}{NLI$_{\text{BART}}$~\cite{Sainz2021NLI}}    & 50.7                  & 48.7                  & {\ul 49.7}                                  & 59.5                  & 34.9                  & 44.0                                     & 49.1                  & 51.8                  & 50.4                                       & 21.6                  & 23.7                  & 22.6                                        & 41.7                                        \\
% \multicolumn{2}{l|}{NLI$_{\text{RoBERTa}}$~\cite{Sainz2021NLI}} & 35.9                  & 68.4                  & 47.1                                        & 52.3                  & 67.0                  & 58.7                                     & 37.2                  & 75.9                  & 49.9                                       & 17.6                  & 20.9                  & 19.1                                        & 43.7                                        \\
% \multicolumn{2}{l|}{NLI$_{\text{DeBERTa}}$~\cite{Sainz2021NLI}} & 52.1                  & 47.0                  & 49.4                                        & 71.7                  & 58.3                  & \textbf{64.3}                            & 52.8                  & 46.8                  & 49.6                                       & 22.0                  & 25.7                  & 23.7                                        & 46.8                                        \\
% \multicolumn{2}{l|}{SuRE$_\text{BART}$~\cite{Lu2022SuRE}}       & 13.1                  & 45.7                  & 20.4                                        & 17.9                  & 34.6                  & 23.6                                     & 14.1                  & 52.3                  & 22.2                                       & 0.0                   & 0.0                   & 0.0                                         & 16.5                                        \\
% \multicolumn{2}{l|}{SuRE$_\text{PEGASUS}$~\cite{Lu2022SuRE}}    & 13.8                  & 51.7                  & 21.8                                        & 16.6                  & 34.6                  & 22.4                                     & 13.5                  & 54.1                  & 21.6                                       & 0.0                   & 0.0                   & 0.0                                         & 16.4                                        \\ \midrule
% \multirow{2}{*}{text-davinci-002}            & Vanilla          & 31.2                  & 73.1                  & 43.7                                        & 44.1                  & 76.3                  & 55.9                                     & 30.2                  & 76.8                  & 43.3                                       & 31.4                  & 28.8                  & 30.1                                        & 43.2                                        \\
%                                              & QA4RE        & 35.6                  & 68.4                  & 46.8 (\textcolor{ForestGreen}{$+$3.1})           & 46.4                  & 72.4                  & 56.5 (\textcolor{ForestGreen}{$+$0.6})        & 35.7                  & 76.8                  & 48.8 (\textcolor{ForestGreen}{$+$5.4})          & 29.4                  & 34.3                  & 31.6  (\textcolor{ForestGreen}{$+$1.5})          & 45.9  (\textcolor{ForestGreen}{$+$2.7})          \\
% \multirow{2}{*}{code-davinci-002}            & Vanilla          & 27.2                  & 70.1                  & 39.2                                        & 42.7                  & 70.4                  & 53.1                                     & 27.5                  & 77.7                  & 40.6                                       & 27.2                  & 25.6                  & 26.4                                        & 39.8                                        \\
%                                              & QA4RE        & 37.7                  & 65.4                  & 47.8 (\textcolor{ForestGreen}{$+$8.6})           & 48.0                  & 74.0                  & 58.2  (\textcolor{ForestGreen}{$+$5.1})       & 31.7                  & 65.5                  & 42.7  (\textcolor{ForestGreen}{$+$2.1})         & 25.2                  & 29.2                  & 27.0  (\textcolor{ForestGreen}{$+$0.6})          & 43.9  (\textcolor{ForestGreen}{$+$4.1})          \\
% \multirow{2}{*}{text-davinci-003}            & Vanilla          & 36.9                  & 68.8                  & 48.1                                        & 49.7                  & 62.2                  & 55.3                                     & 38.2                  & 76.8                  & {\ul 51.0}                                 & 33.2                  & 39.3                  & {\ul 36.0}                                  & {\ul 47.6}                                  \\
%                                              & QA4RE        & 47.7                  & 78.6                  & \textbf{59.4} (\textcolor{ForestGreen}{$+$11.3}) & 56.2                  & 67.2                  & {\ul 61.2}  (\textcolor{ForestGreen}{$+$5.9}) & 46.0                  & 83.6                  & \textbf{59.4} (\textcolor{ForestGreen}{$+$8.4}) & 41.7                  & 45.0                  & \textbf{43.3}  (\textcolor{ForestGreen}{$+$7.3}) & \textbf{55.8}  (\textcolor{ForestGreen}{$+$8.2}) \\ \bottomrule
% \end{tabular}

% Version 2
\begin{tabular}{ll|lllllllllllll}
\toprule
% \multicolumn{2}{c|}{\multirow{2}{*}{Datasets}}                  & \multicolumn{3}{c}{\textbf{TACRED}}                                                         & \multicolumn{3}{c}{\textbf{RE-TACRED}}                                                   & \multicolumn{3}{c}{\textbf{TACREV}}                                                        & \multicolumn{3}{c}{\textbf{SemEval}}                                                        & \multicolumn{1}{c}{\textbf{Average}}            \\
% \multicolumn{2}{c|}{}                                           & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                      & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                   & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                     & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                      & \multicolumn{1}{c}{F1}             \\ \midrule
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Methods}}}                  & \multicolumn{3}{l}{$\mspace{24mu}$ \textbf{TACRED}}                                                         & \multicolumn{3}{l}{$\mspace{13mu}$ \textbf{RETACRED}}                                                   & \multicolumn{3}{l}{$\mspace{24mu}$ \textbf{TACREV}}                                                        & \multicolumn{3}{l}{$\mspace{24mu}$ \textbf{SemEval}}                                                        & \multicolumn{1}{l}{$\mspace{1mu}$\textbf{Avg.}}            \\
\multicolumn{2}{c|}{}                                           & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                      & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                   & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                     & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                      & \multicolumn{1}{l}{$\mspace{3mu}$ F1}             \\ \midrule
\multicolumn{2}{l|}{NLI$_{\text{BART}}$}    & 42.6                  & 65.0                  & 51.4                                        & 59.5                  & 34.9                  & 44.0                                     & 44.0                  & 74.6                  & 55.3                                       & 21.6                  & 23.7                  & 22.6                                        & 43.3                                        \\
\multicolumn{2}{l|}{NLI$_{\text{RoBERTa}}$} & 37.1                  & 76.9                  & 50.1                                        & 52.3                  & 67.0                  & 58.7                                     & 37.1                  & 83.6                  & 51.4                                       & 17.6                  & 20.9                  & 19.1                                        & 44.8                                        \\
\multicolumn{2}{l|}{NLI$_{\text{DeBERTa}}$} & 42.9                  & 76.9                  & {\ul 55.1}                                  & 71.7                  & 58.3                  & \textbf{64.3}                            & 43.3                  & 84.6                  & {\ul 57.2}                                 & 22.0                  & 25.7                  & 23.7                                        & {\ul 50.1}                                  \\

\multicolumn{2}{l|}{SuRE$_\text{BART}$}       & 13.1                  & 45.7                  & 20.4                                        & 17.9                  & 34.6                  & 23.6                                     & 14.1                  & 52.3                  & 22.2                                       & 0.0                   & 0.0                   & 0.0                                         & 16.5                                        \\
\multicolumn{2}{l|}{SuRE$_\text{PEGASUS}$}    & 13.8                  & 51.7                  & 21.8                                        & 16.6                  & 34.6                  & 22.4                                     & 13.5                  & 54.1                  & 21.6                                       & 0.0                   & 0.0                   & 0.0                                         & 16.4                                        \\ \midrule
\multirow{2}{*}{code-002}            & Vanilla          & 27.2                  & 70.1                  & 39.2                                        & 42.7                  & 70.4                  & 53.1                                     & 27.5                  & 77.7                  & 40.6                                       & 27.2                  & 25.6                  & 26.4                                        & 39.8                                        \\
                                             & QA4RE        & 37.7                  & 65.4                  & 47.8 (\textcolor{ForestGreen}{$+$8.6})           & 48.0                  & 74.0                  & 58.2  (\textcolor{ForestGreen}{$+$5.1})       & 31.7                  & 65.5                  & 42.7  (\textcolor{ForestGreen}{$+$2.1})         & 25.2                  & 29.2                  & 27.0  (\textcolor{ForestGreen}{$+$0.6})          & 43.9  (\textcolor{ForestGreen}{$+$4.1})          \\
\multirow{2}{*}{text-002}            & Vanilla          & 31.2                  & 73.1                  & 43.7                                        & 44.1                  & 76.3                  & 55.9                                     & 30.2                  & 76.8                  & 43.3                                       & 31.4                  & 28.8                  & 30.1                                        & 43.2                                        \\
                                             & QA4RE        & 35.6                  & 68.4                  & 46.8 (\textcolor{ForestGreen}{$+$3.1})           & 46.4                  & 72.4                  & 56.5 (\textcolor{ForestGreen}{$+$0.6})        & 35.7                  & 76.8                  & 48.8 (\textcolor{ForestGreen}{$+$5.4})          & 29.4                  & 34.3                  & 31.6  (\textcolor{ForestGreen}{$+$1.5})          & 45.9  (\textcolor{ForestGreen}{$+$2.7})          \\
% \multirow{2}{*}{code-davinci-002}            & Vanilla          & 27.2                  & 70.1                  & 39.2                                        & 42.7                  & 70.4                  & 53.1                                     & 27.5                  & 77.7                  & 40.6                                       & 27.2                  & 25.6                  & 26.4                                        & 39.8                                        \\
%                                              & QA4RE        & 37.7                  & 65.4                  & 47.8 (\textcolor{ForestGreen}{$+$8.6})           & 48.0                  & 74.0                  & 58.2  (\textcolor{ForestGreen}{$+$5.1})       & 31.7                  & 65.5                  & 42.7  (\textcolor{ForestGreen}{$+$2.1})         & 25.2                  & 29.2                  & 27.0  (\textcolor{ForestGreen}{$+$0.6})          & 43.9  (\textcolor{ForestGreen}{$+$4.1})          \\
\multirow{2}{*}{text-003}            & Vanilla          & 36.9                  & 68.8                  & 48.1                                        & 49.7                  & 62.2                  & 55.3                                     & 38.2                  & 76.8                  & 51.0                                 & 33.2                  & 39.3                  & {\ul 36.0}                                  & 47.6                               \\
                                             & QA4RE        & 47.7                  & 78.6                  & \textbf{59.4} (\textcolor{ForestGreen}{$+$11.3}) & 56.2                  & 67.2                  & {\ul 61.2}  (\textcolor{ForestGreen}{$+$5.9}) & 46.0                  & 83.6                  & \textbf{59.4} (\textcolor{ForestGreen}{$+$8.4}) & 41.7                  & 45.0                  & \textbf{43.3}  (\textcolor{ForestGreen}{$+$7.3}) & \textbf{55.8}  (\textcolor{ForestGreen}{$+$8.2}) \\ \bottomrule
\end{tabular}
}

% OrangeRed
% \caption{}
\caption{Experimental results on four RE datasets (\%). 
We omit the `davinci' within the names of LLMs.  We mark the best results in \textbf{bold}, the second-best {\ul underlined}, and F1 improvement of our QA4RE over vanilla RE in \textcolor{ForestGreen}{green}.}
% \caption{Experimental results on four RE datasets (\%). 
% We omit the `davinci' within the names of GPT-3.5 Series LLMs and ChatGPT refers to gpt-3.5-turbo-0301.
% We mark the best results in \textbf{bold}, the second-best {\ul underlined}, and F1 improvement of our QA4RE over vanilla RE in \textcolor{ForestGreen}{green}.}
% \vspace{-15pt}
\vspace{-5pt}
\label{tab:main-table}

\end{table*}

==> tables/zero-shot-main.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
% \small
\centering
\resizebox{\textwidth}{!}{
% \begin{tabular}{ll|lllllllllllll}
% \toprule
% % \multicolumn{2}{c|}{\multirow{2}{*}{Datasets}}                  & \multicolumn{3}{c}{\textbf{TACRED}}                                                         & \multicolumn{3}{c}{\textbf{RE-TACRED}}                                                   & \multicolumn{3}{c}{\textbf{TACREV}}                                                        & \multicolumn{3}{c}{\textbf{SemEval}}                                                        & \multicolumn{1}{c}{\textbf{Average}}            \\
% % \multicolumn{2}{c|}{}                                           & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                      & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                   & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                     & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                      & \multicolumn{1}{c}{F1}             \\ \midrule
% \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Methods}}}                  & \multicolumn{3}{l}{$\mspace{24mu}$ \textbf{TACRED}}                                                         & \multicolumn{3}{l}{$\mspace{10mu}$ \textbf{RE-TACRED}}                                                   & \multicolumn{3}{l}{$\mspace{24mu}$ \textbf{TACREV}}                                                        & \multicolumn{3}{l}{$\mspace{24mu}$ \textbf{SemEval}}                                                        & \multicolumn{1}{l}{$\mspace{1mu}$\textbf{Avg.}}            \\
% \multicolumn{2}{c|}{}                                           & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                      & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                   & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                     & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                      & \multicolumn{1}{l}{$\mspace{3mu}$ F1}             \\ \midrule
% \multicolumn{2}{l|}{NLI$_{\text{BART}}$~\cite{Sainz2021NLI}}    & 50.7                  & 48.7                  & {\ul 49.7}                                  & 59.5                  & 34.9                  & 44.0                                     & 49.1                  & 51.8                  & 50.4                                       & 21.6                  & 23.7                  & 22.6                                        & 41.7                                        \\
% \multicolumn{2}{l|}{NLI$_{\text{RoBERTa}}$~\cite{Sainz2021NLI}} & 35.9                  & 68.4                  & 47.1                                        & 52.3                  & 67.0                  & 58.7                                     & 37.2                  & 75.9                  & 49.9                                       & 17.6                  & 20.9                  & 19.1                                        & 43.7                                        \\
% \multicolumn{2}{l|}{NLI$_{\text{DeBERTa}}$~\cite{Sainz2021NLI}} & 52.1                  & 47.0                  & 49.4                                        & 71.7                  & 58.3                  & \textbf{64.3}                            & 52.8                  & 46.8                  & 49.6                                       & 22.0                  & 25.7                  & 23.7                                        & 46.8                                        \\
% \multicolumn{2}{l|}{SuRE$_\text{BART}$~\cite{Lu2022SuRE}}       & 13.1                  & 45.7                  & 20.4                                        & 17.9                  & 34.6                  & 23.6                                     & 14.1                  & 52.3                  & 22.2                                       & 0.0                   & 0.0                   & 0.0                                         & 16.5                                        \\
% \multicolumn{2}{l|}{SuRE$_\text{PEGASUS}$~\cite{Lu2022SuRE}}    & 13.8                  & 51.7                  & 21.8                                        & 16.6                  & 34.6                  & 22.4                                     & 13.5                  & 54.1                  & 21.6                                       & 0.0                   & 0.0                   & 0.0                                         & 16.4                                        \\ \midrule
% \multirow{2}{*}{text-davinci-002}            & Vanilla          & 31.2                  & 73.1                  & 43.7                                        & 44.1                  & 76.3                  & 55.9                                     & 30.2                  & 76.8                  & 43.3                                       & 31.4                  & 28.8                  & 30.1                                        & 43.2                                        \\
%                                              & QA4RE        & 35.6                  & 68.4                  & 46.8 (\textcolor{ForestGreen}{$+$3.1})           & 46.4                  & 72.4                  & 56.5 (\textcolor{ForestGreen}{$+$0.6})        & 35.7                  & 76.8                  & 48.8 (\textcolor{ForestGreen}{$+$5.4})          & 29.4                  & 34.3                  & 31.6  (\textcolor{ForestGreen}{$+$1.5})          & 45.9  (\textcolor{ForestGreen}{$+$2.7})          \\
% \multirow{2}{*}{code-davinci-002}            & Vanilla          & 27.2                  & 70.1                  & 39.2                                        & 42.7                  & 70.4                  & 53.1                                     & 27.5                  & 77.7                  & 40.6                                       & 27.2                  & 25.6                  & 26.4                                        & 39.8                                        \\
%                                              & QA4RE        & 37.7                  & 65.4                  & 47.8 (\textcolor{ForestGreen}{$+$8.6})           & 48.0                  & 74.0                  & 58.2  (\textcolor{ForestGreen}{$+$5.1})       & 31.7                  & 65.5                  & 42.7  (\textcolor{ForestGreen}{$+$2.1})         & 25.2                  & 29.2                  & 27.0  (\textcolor{ForestGreen}{$+$0.6})          & 43.9  (\textcolor{ForestGreen}{$+$4.1})          \\
% \multirow{2}{*}{text-davinci-003}            & Vanilla          & 36.9                  & 68.8                  & 48.1                                        & 49.7                  & 62.2                  & 55.3                                     & 38.2                  & 76.8                  & {\ul 51.0}                                 & 33.2                  & 39.3                  & {\ul 36.0}                                  & {\ul 47.6}                                  \\
%                                              & QA4RE        & 47.7                  & 78.6                  & \textbf{59.4} (\textcolor{ForestGreen}{$+$11.3}) & 56.2                  & 67.2                  & {\ul 61.2}  (\textcolor{ForestGreen}{$+$5.9}) & 46.0                  & 83.6                  & \textbf{59.4} (\textcolor{ForestGreen}{$+$8.4}) & 41.7                  & 45.0                  & \textbf{43.3}  (\textcolor{ForestGreen}{$+$7.3}) & \textbf{55.8}  (\textcolor{ForestGreen}{$+$8.2}) \\ \bottomrule
% \end{tabular}


\begin{tabular}{ll|lllllllllllll}
\toprule
% \multicolumn{2}{c|}{\multirow{2}{*}{Datasets}}                  & \multicolumn{3}{c}{\textbf{TACRED}}                                                         & \multicolumn{3}{c}{\textbf{RE-TACRED}}                                                   & \multicolumn{3}{c}{\textbf{TACREV}}                                                        & \multicolumn{3}{c}{\textbf{SemEval}}                                                        & \multicolumn{1}{c}{\textbf{Average}}            \\
% \multicolumn{2}{c|}{}                                           & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                      & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                   & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                     & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1}                      & \multicolumn{1}{c}{F1}             \\ \midrule
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Methods}}}                  & \multicolumn{3}{l}{$\mspace{24mu}$ \textbf{TACRED}}                                                         & \multicolumn{3}{l}{$\mspace{10mu}$ \textbf{RE-TACRED}}                                                   & \multicolumn{3}{l}{$\mspace{24mu}$ \textbf{TACREV}}                                                        & \multicolumn{3}{l}{$\mspace{24mu}$ \textbf{SemEval}}                                                        & \multicolumn{1}{l}{$\mspace{1mu}$\textbf{Avg.}}            \\
\multicolumn{2}{c|}{}                                           & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                      & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                   & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                     & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{l}{$\mspace{3mu}$ F1}                      & \multicolumn{1}{l}{$\mspace{3mu}$ F1}             \\ \midrule
\multicolumn{2}{l|}{NLI$_{\text{BART}}$~\cite{Sainz2021NLI}}    & 42.6                  & 65.0                  & 51.4                                        & 59.5                  & 34.9                  & 44.0                                     & 44.0                  & 74.6                  & 55.3                                       & 21.6                  & 23.7                  & 22.6                                        & 43.3                                        \\
\multicolumn{2}{l|}{NLI$_{\text{RoBERTa}}$~\cite{Sainz2021NLI}} & 37.1                  & 76.9                  & 50.1                                        & 52.3                  & 67.0                  & 58.7                                     & 37.1                  & 83.6                  & 51.4                                       & 17.6                  & 20.9                  & 19.1                                        & 44.8                                        \\
\multicolumn{2}{l|}{NLI$_{\text{DeBERTa}}$~\cite{Sainz2021NLI}} & 42.9                  & 76.9                  & {\ul 55.1}                                  & 71.7                  & 58.3                  & \textbf{64.3}                            & 43.3                  & 84.6                  & {\ul 57.2}                                 & 22.0                  & 25.7                  & 23.7                                        & {\ul 50.1}                                  \\

\multicolumn{2}{l|}{SuRE$_\text{BART}$~\cite{Lu2022SuRE}}       & 13.1                  & 45.7                  & 20.4                                        & 17.9                  & 34.6                  & 23.6                                     & 14.1                  & 52.3                  & 22.2                                       & 0.0                   & 0.0                   & 0.0                                         & 16.5                                        \\
\multicolumn{2}{l|}{SuRE$_\text{PEGASUS}$~\cite{Lu2022SuRE}}    & 13.8                  & 51.7                  & 21.8                                        & 16.6                  & 34.6                  & 22.4                                     & 13.5                  & 54.1                  & 21.6                                       & 0.0                   & 0.0                   & 0.0                                         & 16.4                                        \\ \midrule
% \multirow{2}{*}{davinci}                     & Vanilla          & 13.6                  & 51.3                  & 21.5                                        & 31.7                  & 67.4                  & 43.1                                     & 12.1                  & 49.1                  & 19.4                                       & 11.8                  & 9.5                   & 10.5                                        & 23.6                                        \\
%                                              & QA4RE            & 12.6                  & 53.9                  & 20.5 (\textcolor{BrickRed}{$-$1.0})             & 33.8                  & 76.8                  & 47.0 (\textcolor{ForestGreen}{$+$3.9})        & 12.6                  & 56.8                  & 20.6 (\textcolor{ForestGreen}{$+$1.2})          & 6.0                   & 7.1                   & 6.5 (\textcolor{BrickRed}{$-$4.0})              & 23.7 (\textcolor{ForestGreen}{$+$0.1})           \\
% \multirow{2}{*}{text-davinci-001}            & Vanilla          & 14.3                  & 58.1                  & 23.0                                        & 28.2                  & 62.9                  & 39.0                                     & 13.0                  & 57.3                  & 21.3                                       & 5.7                   & 6.5                   & 6.1                                         & 22.3                                        \\
%                                              & QA4RE            & 11.1                  & 24.4                  & 15.3 (\textcolor{BrickRed}{$-$7.7})             & 14.4                  & 26.0                  & 18.5 (\textcolor{BrickRed}{$-$20.5})         & 10.6                  & 24.1                  & 14.7 (\textcolor{BrickRed}{$-$6.6})            & 10.1                  & 12.0                  & 11.0 (\textcolor{ForestGreen}{$+$4.9})           & 14.9 (\textcolor{BrickRed}{$-$7.4})             \\
\multirow{2}{*}{code-davinci-002}            & Vanilla          & 27.2                  & 70.1                  & 39.2                                        & 42.7                  & 70.4                  & 53.1                                     & 27.5                  & 77.7                  & 40.6                                       & 27.2                  & 25.6                  & 26.4                                        & 39.8                                        \\
                                             & QA4RE        & 37.7                  & 65.4                  & 47.8 (\textcolor{ForestGreen}{$+$8.6})           & 48.0                  & 74.0                  & 58.2  (\textcolor{ForestGreen}{$+$5.1})       & 31.7                  & 65.5                  & 42.7  (\textcolor{ForestGreen}{$+$2.1})         & 25.2                  & 29.2                  & 27.0  (\textcolor{ForestGreen}{$+$0.6})          & 43.9  (\textcolor{ForestGreen}{$+$4.1})          \\
\multirow{2}{*}{text-davinci-002}            & Vanilla          & 31.2                  & 73.1                  & 43.7                                        & 44.1                  & 76.3                  & 55.9                                     & 30.2                  & 76.8                  & 43.3                                       & 31.4                  & 28.8                  & 30.1                                        & 43.2                                        \\
                                             & QA4RE        & 35.6                  & 68.4                  & 46.8 (\textcolor{ForestGreen}{$+$3.1})           & 46.4                  & 72.4                  & 56.5 (\textcolor{ForestGreen}{$+$0.6})        & 35.7                  & 76.8                  & 48.8 (\textcolor{ForestGreen}{$+$5.4})          & 29.4                  & 34.3                  & 31.6  (\textcolor{ForestGreen}{$+$1.5})          & 45.9  (\textcolor{ForestGreen}{$+$2.7})          \\
% \multirow{2}{*}{code-davinci-002}            & Vanilla          & 27.2                  & 70.1                  & 39.2                                        & 42.7                  & 70.4                  & 53.1                                     & 27.5                  & 77.7                  & 40.6                                       & 27.2                  & 25.6                  & 26.4                                        & 39.8                                        \\
%                                              & QA4RE        & 37.7                  & 65.4                  & 47.8 (\textcolor{ForestGreen}{$+$8.6})           & 48.0                  & 74.0                  & 58.2  (\textcolor{ForestGreen}{$+$5.1})       & 31.7                  & 65.5                  & 42.7  (\textcolor{ForestGreen}{$+$2.1})         & 25.2                  & 29.2                  & 27.0  (\textcolor{ForestGreen}{$+$0.6})          & 43.9  (\textcolor{ForestGreen}{$+$4.1})          \\
\multirow{2}{*}{text-davinci-003}            & Vanilla          & 36.9                  & 68.8                  & 48.1                                        & 49.7                  & 62.2                  & 55.3                                     & 38.2                  & 76.8                  & 51.0                                 & 33.2                  & 39.3                  & {\ul 36.0}                                  & 47.6                               \\
                                             & QA4RE        & 47.7                  & 78.6                  & \textbf{59.4} (\textcolor{ForestGreen}{$+$11.3}) & 56.2                  & 67.2                  & {\ul 61.2}  (\textcolor{ForestGreen}{$+$5.9}) & 46.0                  & 83.6                  & \textbf{59.4} (\textcolor{ForestGreen}{$+$8.4}) & 41.7                  & 45.0                  & \textbf{43.3}  (\textcolor{ForestGreen}{$+$7.3}) & \textbf{55.8}  (\textcolor{ForestGreen}{$+$8.2}) \\ \bottomrule
\end{tabular}
}

% \caption{}
\caption{Experimental results on 4 RE datasets (\%). We mark the best results in \textbf{bold}, the second-best {\ul underlined}, and the F1 improvements of our QA framework over Vanilla RE in \textcolor{ForestGreen}{green}.}
\vspace{-15pt}
\label{tab:main-table}

\end{table*}
